Complex and Adaptive Dynamical Systems: A Primer

An thorough introduction is given at an introductory level to the field of quantitative complex system science, with special emphasis on emergence in dynamical systems based on network topologies. Subjects treated include graph theory and small-world networks, a generic introduction to the concepts of dynamical system theory, random Boolean networks, cellular automata and self-organized criticality, the statistical modeling of Darwinian evolution, synchronization phenomena and an introduction to the theory of cognitive systems. It inludes chapter on Graph Theory and Small-World Networks, Chaos, Bifurcations and Diffusion, Complexity and Information Theory, Random Boolean Networks, Cellular Automata and Self-Organized Criticality, Darwinian evolution, Hypercycles and Game Theory, Synchronization Phenomena and Elements of Cognitive System Theory.

==> aboutThisBook_inp.tex <==
%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%
%\addcontentsline{toc}{chapter}{\ About This Book}
                        % set the headings for the tableofcontents
\chaptermark{About this Book}
                        % set the headers manually

%\chapter*{\small}
%\vspace{-11ex}
\markboth{About this Book}{About this Book}


\chapter*{About this Book}

%\centerline{\LARGE\bf About This Book}
%\bigskip \bigskip \bigskip \bigskip

\runinhead{From Evolving Networks to Cognitive
Systems Theory} This textbook covers a wide range
of concepts, notions and phenomena of a truly interdisciplinary
subject of rapidly growing importance. Complex system theory deals
with dynamical systems containing a very large number of variables,
showing a plethora of emergent features, arising in a broad range of
contexts. A central focus of these notes is the notion of complexity
arising within evolving and dynamical network structures, such as
the gene expression networks at the basis of all living, adaptive
ecological networks or neural networks for cognitive information
\nobreak processing.

Complex systems theory ultimately forms the basis
of our long-standing quest for exploring and
understanding cognitive systems in general and our brain in
particular -- the mammalian brain is probably the most complex of
all adaptive networks known to humanity.

\runinhead{Readership and Preconditions} 
This primer is intended for graduate students or 
scientists from natural sciences, engineering or 
neuroscience. Technically, the reader should have 
a basic knowledge of ordinary and partial 
differential equations and of probability distributions.
This textbook is suitable both for studies in conjunction with
teaching courses as well as for the individual
reader.

\runinhead{Course Material and the Modular Approach}
When used for teaching, this primer is suitable 
for a course running over 40--60 lecture hours, 
depending on the pace and on the number of chapters 
covered. Essentially all mathematical transformations
are performed on a step-by-step basis and in general 
the reader should have no problem following the 
respective derivations.

Individual chapters, apart from the first three,
having mostly introductory character, may be skipped
whenever time considerations demand it. I have followed 
a basic modular approach and the individual chapters 
are, as far as possible, independent of each other.
Notwithstanding, cross references between the different 
chapters are included throughout the text, since 
interrelations between distinct topics are helpful 
for a thorough understanding.

\runinhead{Style} 
This interdisciplinary primer sets a high value
on conveying concepts and notions within their
respective mathematical settings. Believing that 
a concise style helps the reader to go through 
the material I mostly abstained from long text 
passages with general background explanations or 
philosophical considerations. Widespread
use has been made of paragraph headings, with the
intention to facilitate scientific reading in
this way.

\enlargethispage{6pt}

\runinhead{A Primer to Scientific Common-Sense Knowledge} 
To a certain extent one can regard this textbook as a
primer to a wide range of scientific common-sense \nobreak knowledge
regarding complex systems. Basic knowledge about life's
organizational principles, to give an example, such as the notion of
\qut{life at the edge of chaos}, is important in today's world
to an educated scientist. Other areas of scientific
common-sense knowledge discussed in this primer include network
theory, which has \nobreak applications ranging from social networks
to gene expression networks, the fundamentals of evolution,
cognitive systems theory, as well as the basic principles
of dynamical systems and information theory.

\runinhead{Content} All of the chapters making up this book 
deal with a subject worth devoting an entire course to.
This book addresses readers interested in multidisciplinary 
aspects; I have consequently tried to present succinct 
expositions of the fundamental notions and concepts on 
the basis of the subjects treated in the individual chapters.
%
\begin{description}[1.]

\item[1.] {\em Graph Theory and Small-World Networks} \\
      Networks, ranging from neural networks, social networks,
      ecological networks to gene expression networks,
      are at the basis of many complex systems. Networks tend to
      be adaptive and evolving. Network theory is therefore
      a prerequisite for a thorough understanding of
      adaptive and/or complex systems.

\item[2.] {\em Chaos, Bifurcations and Diffusion} \\
      This chapter introduces basic notions of dynamical
      {systems} theory, such as attractors, bifurcations,
      deterministic chaos, diffusion and stochastic
      resonances, many of which are used throughout these notes.
      Complexity emergent from dynamical systems containing
      many variables, the central theme of this \nobreak textbook,
      is ultimately based on the concepts of classical
      dynamical {systems} theory, treated in this chapter,
      which deals with differential equations involving
      a \nobreak handful of variables.

\item[3.] {\em Complexity and Information Theory} \\
      Information theory provides the basis for statistical
      analysis and time-series characterization, providing
      powerful concepts likes the Shannon entropy and mutual
      information. This chapter will also provide a critical
      assessment of measures proposed to quantify the degree
      of complexity of dynamical systems.

\item[4.] {\em Random Boolean Networks} \\
      A prime model for complex systems with an infinite number
      of variables are random graphs with Boolean variables.
      It allows for the characterization of typical
      dynamical behaviors, e.g.\ \qut{frozen} vs.\ \qut{chaotic},
      which are of relevance in many contexts.
      Of especial importance are random Boolean networks
      for the fundamentals in the realm of life, leading
      to the notion of \qut{life at the edge
      of chaos}.

% \enlargethispage*{12pt}

\item[5.] {\em Cellular Automata and Self-Organized Criticality} \\
      Regular dynamical systems on lattices, the cellular
      automata, allow detailed studies of the dynamics of
      complex systems, a key issue being the organi\-zational
      principle necessary for a dynamical system to show
      the emergent phenomenon of
     \qut{self-organized criticality}.

\item[6.] {\em Darwinian Evolution, Hypercycles and Game Theory} \\
      Evolution of living organisms is, without a doubt,
      the paradigm for an adaptive and complex dynamical
      system, that of interacting species. Key concepts such
      as the \qut{error catastrophe} and \qut{hypercycles} 
      for the prebiotic evolution are discussed within the 
      standard statistical approach, together with the foundations
      of game theory.

\item[7.] {\em Synchronization Phenomena} \\
      When many distinct computational units interact,
      which is a typical situation in complex systems, they might
      evolve synchronously, in phase, or rather independently.
      Synchronization is an issue of wide ranging importance,
      from the outbreak of epidemics to the definition
      of objects in cortical circuits.

\item[8.] {\em Elements of Cognitive Systems Theory} \\
      The most complex of any known dynamical systems, and
      probably also the least understood of all,
      is the brain. It constitutes the biological support
      for the human cognitive system, supposedly the
      most evolved cognitive system known to date.
      Basic principles and important concepts of
      cognitive systems theory are developed in this
      chapter.
\end{description}
%
The basic material and mathematical notions for the course are
developed in the first three chapters. The scientific investigations
of complex systems are just beginning and the subjects chosen 
in Chaps.\ 4--8 are of exemplary importance for this 
rapidly developing field.

\runinhead{Exercises and Suggestions for Individual Studies} 
Towards the end of each individual chapter a selection 
of exercises is presented. Some of them deal with simple
extensions of the material, such as a proof
of a specific formula or the application of a method discussed in
the main text to a different or related problem. Other exercises are
of the form of small work studies, such as the numerical
implementation via a C++ or Maple code of a basic model, with the
objective to obtain a hands-on experience with an
interesting phenomenon from the investigation of the results
obtained from the simulation runs.

This interdisciplinary field is very suitable for 
making an inroad with a basic research project. The 
suggestions for work studies presented in the respective 
exercise sections therefore also serve as guides and 
motivations for a first step towards scientific research 
in this field, which in the end may possibly lead to 
research goals developed by the individual reader. It is 
a highly satisfying experience and is truly recommended.

\runinhead{References and Literature} 
The section \qut{Further Reading} at the end of 
each individual chapter contains references
to standard introductory textbooks and review
articles, and to some articles for further
in-depth studies dealing with selected issues treated within the
respective chapter. Certain original research literature containing
some of the first investigations of phenomena discussed in the
respective chapter is also selectively listed whenever of scientific
or historical interest.

\runinhead{Complexity and Our Future} 
Human society constitutes an adaptive network with 
\qut{intelligent vertices}, us as individuals. On a 
larger scale, intricate interrelations between industrial 
companies, political parties and pressure groups, 
non-governmental organizations (NGOs) of the civil society 
and many other constituent components defy any encompassing
analysis. The complex dynamical system denoted human society will
remain beyond our predictive capacities for many years to
come.

Nevertheless complexity theory represents a fundamental 
tool for long-term modeling and scenario building. A good 
understanding of possible emergent behaviors, of chaotic 
vs.\ regular evolution processes and of stability analysis 
is clearly very helpful when trying to study and model the 
long-term consequences of human actions today. The theory 
of complex and adaptive dynamical systems is a basic tool for
genuine futurology.

\runinhead{The Future of Life and of Our Civilization} 
On a personal note the author believes, in this context, 
that the long-term perspective is of central importance 
as a guideline for global human actions today, in view of 
our capability to change the very face of the earth. We 
are living at a point in history where we, the constituents 
of human society, are not capable of directly controlling 
the global and dynamical developments of this very society, 
an example of what one denotes an emergent behavior -- 
the sum is more than its parts.

We are nevertheless the central actors within human society and the
long-term developments and trends are determined by the underlying
principles, by the long-term guidelines to our actions and planning.
A stronger focus on long-term perspectives and developments, for all
the positive outlook it may provide, for the perils to our
civilization and to life on earth it might reveal, is of central
importance, in the view of the author, at this point in history. The
reader thinking along similar lines is invited to visit the
organization Future 25,\footnote{Or the german counterpart,
{\em Verein Zukunft 25}.} which is dedicated to the 
\qut{future of life and humanity on earth, the 
planets and in the universe}.

\runinhead{Acknowledgements} 
I would like to thank
Tejaswini Dalvi, Florian Dommert, Bernhard Edegger,
Chistoph Herold, Gregor Kaczor, Mathias Linkerhand,
Wolfgang Mader and Dimitrije Markovic for their
help in the preparation of figures and reading, Urs Bergmann,
Christoph Bruder, Dante Cialvo, Florian Greil, Maripola Kolokotsa,
Ludger Santen and DeLiang Wang for comments and
careful reading of the manuscript, Barbara
Drossel and H.G. Schuster for interesting comments, and Roser
Valenti for continuing support.


%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%% general entries for the index
\index{dynamics|see{{\it also} dynamical system}}
\index{graph|see{{\it also} network}}
\index{network|see{{\it also} graph}}
\index{time series analysis|see{{\it also} prediction task}}
\index{action selection|see{decision process}}
\index{associations|see{associative}} 
\index{average|see{mean}}
\index{binary|see{boolean}} 
\index{BTW model|see{sandpile model}}
\index{Conway's game of life|see{game of life}}
\index{damping|see{friction}} 
\index{distribution!degree|see{degree distribution}} 
\index{epistasis|see{epistatic interactions}}
\index{evolutionary game|see{game theory}} 
\index{generating function|see{probability generating function}}
\index{homeostasis|see{homeostatic principles}}
\index{landscape|see{fitness landscape}} 
\index{mean-field approximation|see{mean-field theory}} 
\index{molecular field approximation|see{mean-field theory}} 
\index{self-consistency equation|see{self-consistency condition}} 
\index{simple recurrent network|see{Elman network}} 
\index{synapse|see{synaptic}} 
\index{steady-state solution|see{stationary solution}}
\index{temporal prediction task|see{prediction task}}
\index{trajectory|see{orbit}}
\index{boolean!network|see{boolean network}} 
\index{boolean network!coupling functions|see{coupling ensemble}}
\index{criticality!self-organized|see{self-organized criticality}}
\index{dynamics!transient state|see{transient state dynamics}}
\index{ensemble!coupling functions|see{coupling ensemble}}
\index{graph!random|see{random graph}} 
\index{life!game of|see{game of life}} 
\index{network!{$N$--$K$}|see{Kauffman network}} 
\index{network!Elman|see{Elman network}}
\index{network!Kauffman|see{Kauffman network}}
\index{model!sandpile|see{sandpile model}}
\index{model!BTW|see{sandpile model}}
\index{phase!transition|see{phase transition}}
\index{oscillator!harmonic|see{harmonic oscillator}}
\index{oscillator!relaxation|see{relaxation oscillator}}
\index{time!evolution|see{dynamics}}

\index{Bayesian!PDF|see{probability distribution}}
%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%

